MCFlow: Monte Carlo Flow Models for Data Imputation

We consider the topic of data imputation, a foundational task in machine learning that addresses issues with missing data. To that end, we propose MCFlow, a deep framework for imputation that leverages normalizing flow generative models and Monte Carlo sampling. We address the causality dilemma that arises when training models with incomplete data by introducing an iterative learning scheme which alternately updates the density estimate and the values of the missing entries in the training data. We provide extensive empirical validation of the effectiveness of the proposed method on standard multivariate and image datasets, and benchmark its performance against state-of-the-art alternatives. We demonstrate that MCFlow is superior to competing methods in terms of the quality of the imputed data, as well as with regards to its ability to preserve the semantic structure of the data.

==> one-two-term.tex <==
% \begin{table*}[t]\caption{MCFlow Loss Analysis}\label{tab:one-two-term} 
% \centering
% \setlength\doublerulesep{0.5pt}
% \vspace*{5mm}
% \begin{tabular}{|l|c|c|c|}
% \hline
% RMSE     & Default of Credit Card & Online News Popularity & Letter Recognition \\ \hline
% Weighted Density Estimate & .1354                  & .2021                  & .1186              \\ \hline
% Full Density Estimate & \textbf{.1231}                  & \textbf{.1706}                  & \textbf{.1061}              \\ \hline
% \end{tabular}
% \end{table*}

\begin{table*}[t]\caption{Performance Comparison across Different Loss Term Combinations}\label{tab:loss-analysis} 
\centering
\setlength\doublerulesep{0.5pt}
\vspace*{5mm}
\begin{tabular}{|l|c|c|c|}
\hline
                                     & Default of Credit Card & Online News Popularity & Letter Recognition \\ \hline
$\log$ probability           & .5204               & .6282                & .6677             \\ \hline
$\log$ probability and Jacobian determinant           & .5849                 & .6189                 & .6866             \\ \hline
MSE                             &  .1300                 &  .1773            & .1128                   \\ \hline
MSE and $\log$ probability      & .1354                 & .2021                 & .1186             \\ \hline
Full loss & \textbf{.1231}                  & \textbf{.1706}                  & \textbf{.1061}              \\ \hline
\end{tabular}
\end{table*}

==> reset-table.tex <==


\begin{table*}[t]\caption{Performance Comparison across Scheduling Schemes}\label{tab:reset-table} 
\centering
\setlength\doublerulesep{0.5pt}
\vspace*{5mm}
\begin{tabular}{|l|c|c|c|}
\hline
RMSE              & Default of Credit Card & Online News Popularity & Letter Recognition \\ \hline
Never Reset/Update       & .3071                  & .2920                  & .1379              \\ \hline
Linear Reset/Always Update      &         &         &              \\ \hline
Exponential Reset/Always Update      & .1480         & .2085         & .1265              \\ \hline
Always Reset/Update      & .1567                  & .1944                  & .1251              \\ \hline
Linear Reset/Update      & \textbf{.1213}         & \textbf{.1678}         & .1155              \\ \hline
Exponential Reset/Update & .1231                  & .1706                  & \textbf{.1061}     \\ \hline
\end{tabular}
\end{table*}

